ReDS: A Framework for Reputation-Enhanced DHTs

Distributed Hash Tables (DHTs) such as Chord and Kademlia offer an efficient solution for locating resources in peer-to-peer networks. Unfortunately, malicious nodes along a lookup path can easily subvert such queries. Several systems, including Halo (based on Chord) and Kad (based on Kademlia), mitigate such attacks by using a combination of redundancy and diversity in the paths taken by redundant lookup queries. Much greater assurance can be provided, however. We describe Reputation for Directory Services (ReDS), a framework for enhancing lookups in redundant DHTs by tracking how well other nodes service lookup requests. We describe how the ReDS technique can be applied to virtually any redundant DHT including Halo and Kad. We also study the collaborative identification and removal of bad lookup paths in a way that does not rely on the sharing of reputation scores --- we show that such sharing is vulnerable to attacks that make it unsuitable for most applications of ReDS. Through extensive simulations we demonstrate that ReDS improves lookup success rates for Halo and Kad by 80% or more over a wide range of conditions, even against strategic attackers attempting to game their reputation scores and in the presence of node churn.

==> graphs/Gnuplot/plot <==
set terminal postscript eps enhanced color 18
set datafile separator "\t"
set xlabel "Colluding fraction" 
set ylabel "Locate failure rate"

#set xr [0:0.5]  
set yr [0:.8]
#set key .25,.6  

set output "set1_20.eps"

plot \
'norepSet1.txt' using 1:2 with line title 'Halo' lw 4 ,\
'aboostSet1.txt' using 1:2 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:2 with line title 'Collaborative' lw 4

set output "set1_20-std.eps"

plot \
'norepSet1.txt' using 1:2 with line title 'Halo' lw 4 ,\
'aboostSet1.txt' using 1:2 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:2 with line title 'Collaborative' lw 4,\
'norepSet1.txt' using 1:2:5 with errorbars notitle lt 1 lw 4 ,\
'aboostSet1.txt' using 1:2:5 with errorbars notitle lt 2 lw 4 ,\
'collabSet1.txt' using 1:2:5 with errorbars notitle lt 3 lw 4 

set output "set1_100.eps"

plot \
'norepSet1.txt' using 1:4 with line title 'Halo' lw 4,\
'aboostSet1.txt' using 1:4 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:4 with line title 'Collaborative' lw 4

set output "set1_100-std.eps"

plot \
'norepSet1.txt' using 1:4 with line title 'Halo' lw 4,\
'aboostSet1.txt' using 1:4 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:4 with line title 'Collaborative' lw 4,\
'norepSet1.txt' using 1:4:7 with errorbars notitle lt 1 lw 4 ,\
'aboostSet1.txt' using 1:4:7 with errorbars notitle lt 2 lw 4 ,\
'collabSet1.txt' using 1:4:7 with errorbars notitle lt 3 lw 4 

set output "set1_50.eps"

plot \
'norepSet1.txt' using 1:3 with line title 'Halo' lw 4 ,\
'aboostSet1.txt' using 1:3 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:3 with line title 'Collaborative' lw 4


set output "set1_50-std.eps"

plot \
'norepSet1.txt' using 1:3 with line title 'Halo' lw 4 ,\
'aboostSet1.txt' using 1:3 with line title 'A-Boost' lw 4,\
'collabSet1.txt' using 1:3 with line title 'Collaborative' lw 4,\
'norepSet1.txt' using 1:3:6 with errorbars notitle lt 1 lw 4 ,\
'aboostSet1.txt' using 1:3:6 with errorbars notitle lt 2 lw 4 ,\
'collabSet1.txt' using 1:3:6 with errorbars notitle lt 3 lw 4 



set output "set4_100.eps"
plot \
'set4_100.txt' using 1:2 with line title '100 training' lw 4,\
'set4_100.txt' using 1:3 with line title '200 training' lw 4 ,\
'set4_100.txt' using 1:4 with line title '500 training' lw 4

set output "set4_100-std.eps"
plot \
'set4_100.txt' using 1:2 with line title '100 training' lw 4,\
'set4_100.txt' using 1:3 with line title '200 training' lw 4 ,\
'set4_100.txt' using 1:4 with line title '500 training' lw 4 ,\
'set4_100.txt' using 1:2:5 with errorbars notitle lt 1 lw 4 ,\
'set4_100.txt' using 1:3:6 with errorbars notitle lt 2 lw 4 ,\
'set4_100.txt' using 1:4:7 with errorbars notitle lt 3 lw 4 

set output "set4_50.eps"
plot \
'set4_50.txt' using 1:2 with line title '100 training' lw 4,\
'set4_50.txt' using 1:3 with line title '200 training' lw 4,\
'set4_50.txt' using 1:4 with line title '500 training' lw 4

set output "set4_50-std.eps"
plot \
'set4_50.txt' using 1:2 with line title '100 training' lw 4,\
'set4_50.txt' using 1:3 with line title '200 training' lw 4,\
'set4_50.txt' using 1:4 with line title '200 training' lw 4,\
'set4_50.txt' using 1:2:5 with errorbars notitle lt 1 lw 4 ,\
'set4_50.txt' using 1:3:6 with errorbars notitle lt 2 lw 4,\
'set4_50.txt' using 1:4:7 with errorbars notitle lt 3 lw 4

set xlabel "Attacking percentage"
set output "set2_aboost.eps"
plot \
'aboostSet2.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'aboostSet2.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'aboostSet2.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'aboostSet2.txt' using 1:2 with line title '5% colluding' lw 4

set output "set2_aboost-std.eps"
plot \
'aboostSet2.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'aboostSet2.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'aboostSet2.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'aboostSet2.txt' using 1:2 with line title '5% colluding' lw 4 ,\
'aboostSet2.txt' using 1:5:11 with errorbars notitle lt 1 lw 4 ,\
'aboostSet2.txt' using 1:4:10 with errorbars notitle lt 2 lw 4 ,\
'aboostSet2.txt' using 1:3:9 with errorbars notitle lt 3 lw 4 ,\
'aboostSet2.txt' using 1:2:8 with errorbars notitle lt 4 lw 4 

set output "set2_collab.eps"
plot \
'collabSet2.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'collabSet2.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'collabSet2.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'collabSet2.txt' using 1:2 with line title '5% colluding' lw 4

set output "set2_collab-std.eps"
plot \
'collabSet2.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'collabSet2.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'collabSet2.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'collabSet2.txt' using 1:2 with line title '5% colluding' lw 4,\
'collabSet2.txt' using 1:5:11 with errorbars notitle lt 1 lw 4 ,\
'collabSet2.txt' using 1:4:10 with errorbars notitle lt 2 lw 4 ,\
'collabSet2.txt' using 1:3:9 with errorbars notitle lt 3 lw 4 ,\
'collabSet2.txt' using 1:2:8 with errorbars notitle lt 4 lw 4 

set output "set3_aboost.eps"
plot \
'aboostSet3.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'aboostSet3.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'aboostSet3.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'aboostSet3.txt' using 1:2 with line title '5% colluding' lw 4 

set output "set3_aboost-std.eps"
plot \
'aboostSet3.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'aboostSet3.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'aboostSet3.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'aboostSet3.txt' using 1:2 with line title '5% colluding' lw 4 ,\
'aboostSet3.txt' using 1:5:11 with errorbars notitle lt 1 lw 4 ,\
'aboostSet3.txt' using 1:4:10 with errorbars notitle lt 2 lw 4 ,\
'aboostSet3.txt' using 1:3:9 with errorbars notitle lt 3 lw 4 ,\
'aboostSet3.txt' using 1:2:8 with errorbars notitle lt 4 lw 4 

set output "set3_collab.eps"
plot \
'collabSet3.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'collabSet3.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'collabSet3.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'collabSet3.txt' using 1:2 with line title '5% colluding' lw 4 

set output "set3_collab-std.eps"
plot \
'collabSet3.txt' using 1:5 with line title '20% colluding' lw 4 ,\
'collabSet3.txt' using 1:4 with line title '15% colluding' lw 4 ,\
'collabSet3.txt' using 1:3 with line title '10% colluding' lw 4 ,\
'collabSet3.txt' using 1:2 with line title '5% colluding' lw 4 ,\
'collabSet3.txt' using 1:5:11 with errorbars notitle lt 1 lw 4 ,\
'collabSet3.txt' using 1:4:10 with errorbars notitle lt 2 lw 4 ,\
'collabSet3.txt' using 1:3:9 with errorbars notitle lt 3 lw 4 ,\
'collabSet3.txt' using 1:2:8 with errorbars notitle lt 4 lw 4 

